Learning Deep Visual Object Models From Noisy Web Data: How to Make it Work

Deep networks thrive when trained on large scale data collections. This has given ImageNet a central role in the development of deep architectures for visual object classification. However, ImageNet was created during a specific period in time, and as such it is prone to aging, as well as dataset bias issues. Moving beyond fixed training datasets will lead to more robust visual systems, especially when deployed on robots in new environments which must train on the objects they encounter there. To make this possible, it is important to break free from the need for manual annotators. Recent work has begun to investigate how to use the massive amount of images available on the Web in place of manual image annotations. We contribute to this research thread with two findings: (1) a study correlating a given level of noisily labels to the expected drop in accuracy, for two deep architectures, on two different types of noise, that clearly identifies GoogLeNet as a suitable architecture for learning from Web data; (2) a recipe for the creation of Web datasets with minimal noise and maximum visual variability, based on a visual and natural language processing concept expansion strategy. By combining these two results, we obtain a method for learning powerful deep object models automatically from the Web. We confirm the effectiveness of our approach through object categorization experiments using our Web-derived version of ImageNet on a popular robot vision benchmark database, and on a lifelong object discovery task on a mobile robot.

==> concept_expansion.tex <==
\subsection{Concept Expansion Procedure}
\begin{itemize}
\item start from the list of 1000 classes. Each class can be associated
to multiple synsets/words, take only the first one.
\item use this as input to \emph{mykeyworder}. This is an online engine which
provides us with keywords associated to the given class. (MyKeyworder references language content from Princeton's Wordnet and Moby Thesaurus. MyKeyworder also uses APIs from Google, Shutterstock, Flickr, Text Analysis by AlchemyAPI and several other third parties but is not affiliated with any of these services.)
MyKeyworder will return a list of relevant keywords that is associated with image search queries, semantic concepts and photographic tags.
So the information provided by 
the keyword should be intrinsically visual. Moreover the keywords are sorted 
in terms of frequency and relevance and we take the first 20 keywords as \emph{expanded concepts}.
\item For the original class and for each of the expanded concepts run an
image search on google, flickr and yahoo. 
In all the three cases take the top 200 output images.
We choose 200 because this is the amount of images already considered in previous work \cite{Chatfield12} and it should reasonably give a guarantee against noisy images which generally increase the further we advance with the results.
\item given the images from each class and from all its 20 expansions, remove the duplicates and keep track of the number of images shared between each expansion with reference to the class: in (class,expansion) pairs.
\end{itemize}

\subsection{Experimental tests}
\begin{itemize}
\item {\bf Crap}: This covers the case in which we focus on quantity of images and not on the used search engine or the quality of the images. We use Picsearch which provides very noisy images and we download up to 10000 images per class.
\item {\bf Top}: Use the mykeyworder + concept expansion procedure described above but take only the first images replicating the structure of Imagenet's Large Scale Database (ILSVRC-12)\cite{ILSVRC15}. This in practice means taking the images from the class + the first two/three concept expansions.
\item {\bf Random}: Use the mykeyworder + concept expansion procedure described above. Select a Random subset of images from all obtained images.
\item {\bf Filtered}: Use the mykeyworder + concept expansion procedure, select the images that maximizes the variability of each class using our Variability Maximization method explained below.
\end{itemize}

\subsection{Variability Maximization} 
We want to subselect the expansions that maximize the quality of the final set of data.
We assign to each expansions a score which indicates its quality. 
We suppose that the quality is high if 
\begin{enumerate}
\item  the images of the expansion $e_{ij}$ lay close to the class images $c_i$: small distance $d_{ij}$ evaluated in the fc7 space;
\item   the images of the expansions are not sparse: small standard deviation ($s_{ij}$) of the image set; 
\item   the number of duplicates $dup$ shared by the $(c_i, e_{ij})$ pair is small: insuring variability 
\end{enumerate}
\begin{equation}\label{score_equ}
\large score_{ij}=(d_{ij} \times s_{ij})e^\frac{dup(c_i, e_{ij})} {dup_{max}}
\end{equation}
Using our scoring formula \ref{score_equ} we evaluate each expanded concept a score. This will allow us to choose the concepts that can maximize the variability of the categories. We choose the 5 concepts with the lowest scores which means each category will have images from the class name and 5 \emph{expanded concepts}. Next will be selecting a subset from our pool of images that follows the same structure of Imagenet's.




